Lyapunov-based Safe Policy Optimization for Continuous Control

We study continuous action reinforcement learning problems in which it is crucial that the agent interacts with the environment only through safe policies, i.e.,~policies that do not take the agent to undesirable situations. We formulate these problems as constrained Markov decision processes (CMDPs) and present safe policy optimization algorithms that are based on a Lyapunov approach to solve them. Our algorithms can use any standard policy gradient (PG) method, such as deep deterministic policy gradient (DDPG) or proximal policy optimization (PPO), to train a neural network policy, while guaranteeing near-constraint satisfaction for every policy update by projecting either the policy parameter or the action onto the set of feasible solutions induced by the state-dependent linearized Lyapunov constraints. Compared to the existing constrained PG algorithms, ours are more data efficient as they are able to utilize both on-policy and off-policy data. Moreover, our action-projection algorithm often leads to less conservative policy updates and allows for natural integration into an end-to-end PG training pipeline. We evaluate our algorithms and compare them with the state-of-the-art baselines on several simulated (MuJoCo) tasks, as well as a real-world indoor robot navigation problem, demonstrating their effectiveness in terms of balancing performance and constraint satisfaction. Videos of the experiments can be found in the following link: https://drive.google.com/file/d/1pzuzFqWIE710bE2U6DmS59AfRzqK2Kek/view?usp=sharing.

==> def.tex <==
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\RR}{\mathbb{R}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\R}{r}
\newcommand{\RV}{R}
\newcommand{\Pd}{\mathbb P_\tau}
\newcommand{\Pdx}{\mathbb P_{\text{data,x}}}
\newcommand{\Pdr}{\mathbb P_{\text{data,r}}}

\newcommand{\excise}[1]{}

==> relwork.tex <==
%!TEX root = safety_icml.tex

%\textit{Safety:} In some problems, it is not only important that the policy learned by the agent (that will be deployed) be safe~\citep{amodei2016concrete}, but also crucial that all the policies generated during training (with which the agent interacts with the environment to collect samples) be safe~\citep{achiam2017constrained}. For example, a robot should always avoid taking actions that irrevocably harm its hardware.

\textit{Constrained Markov Decision Processes:}
%The additional constraint cost function gives more flexibility to CMDPs in modeling problems with \emph{trajectory-based} constraints compared to approaches that artificially re-cast the cost of MDPs to enforce the constraints~\citep{regan2009regret}. Under the CMDP framework, we consider a policy to be {\em safe} if it satisfies the cumulative cost constraints.
A common approach to solve CMDPs is to use the Lagrangian method~\citep{altman1998constrained,geibel2005risk} that augments the original objective function with a penalty on constraint violation and computes the saddle-point of the constrained policy optimization via primal-dual method~\citep{chow2017risk}. Although safety is ensured when the policy converges {\em asymptotically}, a major drawback of this approach is that it makes no guarantee with regards to the safety of the policies generated during training. Heuristic algorithms for policy search with safety constraints (e.g.,~\citealt{uchibe2007constrained}) address the issue of safety during training. While some of them work reasonably well in practice, none is theoretically grounded to generate constraint-satisfying policies.

\textit{Constrained Policy Optimization:}
 {\em Constrained policy optimization} (CPO) \citet{achiam2017constrained} extends the trust-region policy optimization (TRPO)~\citep{schulman2015trust} to handle CMDP constraints in a principled way. CPO has promising empirical results in terms scalability, performance, and constraint satisfaction, both during training and after convergence. Yet, CPO has three downsides that the presented method addresses. First, CPO offers no theoretical guarantees, while our method is founded on the Lyapunov stability theory, and had build-in theoretical safety guarantees. Second, CPO is closely connected to TRPO, and policy gradient algorithms that are regularized with relative entropy (such as PPO). It is not clear how it can be combined with algorithms that do not belong to the family of proximal PG algorithms, such as DDPG. Our method  can be applied to more general RL algorithms, including in off-policy settings. We present both safe PPO, and safe DDPG. In fact, as we show in Section \ref{sec:theta_proj}, CPO can be viewed as a special case of Lyapunov-based PG (which is known as SPPO in this paper). Last, CPO is not a \emph{back-propagatable} algorithm, due to the backtracking line-search procedure and the conjugate gradient iterations for computing natural gradient in TRPO. Our algorithms can be trained \emph{end-to-end}, which is crucial for scalable and efficient implementations \citep{hafner2017tensorflow}.

\textit{Lyapunov stability theory and reinforcement learning:}
Lyapunov stability theory has long history in control theory to analyze the stability of dynamical systems~\citep{khalil1996noninear,neely2010stochastic}. Lyapunov functions in RL are used to guarantee closed-loop stability of an agent ~\citet{perkins2002lyapunov,faust-acta-14}. \citet{berkenkamp2017safe} uses Lyapunov functions to guarantee that a model-based RL agent can be brought back to a ``region of attraction'' during exploration. 
Using the theoretical underpinnings of the Lyapunov approach,~\citet{chow2018lyapunov} propose approximate policy and value iteration RL algorithms for discrete action CMDP. However, since their algorithms are value-function-based, applying them to continuous action problems is not straightforward. The present builds on top of the theoretical framework~\citet{chow2018lyapunov}, and produces policy optimization in continuous action CMDP.  

\textit{Safety Layer:}
\citet{dalal2018safe} proposes a safety layer as a solution for constraints that can only be expressed locally. Our method solves more general CMDP problem (with trajectory-based constraints). Our paper provides an elegant recipe (through the use of Lyapunov functions) to adopt the safety layer concept to solve safe RL problems with general trajectory-based constraints using direct \emph{back-propagation}.

